Mandheling: Mixed-Precision On-Device DNN Training with DSP Offloading

This paper proposes Mandheling, the first system that enables highly resource-efficient on-device training by orchestrating the mixed-precision training with on-chip Digital Signal Processing (DSP) offloading. Mandheling fully explores the advantages of DSP in integer-based numerical calculation by four novel techniques: (1) a CPU-DSP co-scheduling scheme to mitigate the overhead from DSP-unfriendly operators; (2) a self-adaptive rescaling algorithm to reduce the overhead of dynamic rescaling in backward propagation; (3) a batch-splitting algorithm to improve the DSP cache efficiency; (4) a DSP-compute subgraph reusing mechanism to eliminate the preparation overhead on DSP. We have fully implemented Mandheling and demonstrate its effectiveness through extensive experiments. The results show that, compared to the state-of-the-art DNN engines from TFLite and MNN, Mandheling reduces the per-batch training time by 5.5$\times$ and the energy consumption by 8.9$\times$ on average. In end-to-end training tasks, Mandheling reduces up to 10.7$\times$ convergence time and 13.1$\times$ energy consumption, with only 1.9%-2.7% accuracy loss compared to the FP32 precision setting.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> algorithm-split-batch.tex <==
\begin{algorithm}[t]
	\small
	\caption{Find the batch splitting point}
	\label{algo:batch-splitting}
	\SetKwFunction{FCompute}{compute}
	\SetKwProg{Fn}{Function}{:}{}
	\SetKwProg{Pn}{Function}{:}{\KwRet}
	
	\KwData{\textit{Model}, \textit{memory\_bydget}}
	\KwResult{split\_plan}
	
	%	comp\_seq = getCompSeqInTopoOrder(profiling)\;
	%	pool = Pool.alloc(comp\_seq, profiling)\;
	Initialize \textit{profiling\_map}, \textit{abnormal\_list} and \textit{potential\_batch\_list} = \{1,2,4,8,16,32,64\}\;
	%	Initialize \textit{exec\_plan} via \textit{comp\_seq} and \textit{pool}\;
	\textit{profiling\_map} $\leftarrow$ Map(); \tcp{\tiny workload -> latency}
	\textit{abnormal\_list} $\leftarrow$ List(0); \tcp{\tiny Layers with abnormally latency growth}
	\textit{split\_plan} $\leftarrow$ List<Tuple>(0); \tcp{\tiny layers and their split numbers}
	
	\ForEach{\normalfont$op_i$ in \textit{Model}}{
		
		\textit{work\_op} $\leftarrow$ getComputationWorkload($op_i$)\;
		\textit{time\_op} $\leftarrow$ profileExecutionLatency($op_i$)\;
		
		\While{\normalfont $iter\_work\_op_j$,  $iter\_time\_op_j$ in \textit{profiling\_map}}{
			
			\If{	\textit{work\_op}  /  \textit{$iter\_work\_op_j$}  < 	\textit{time\_op}  / $iter\_time\_op_j$ }{
				
					\textit{abnormal\_list}.append(\textit{i})\;
			}
			
		}
		\textit{profiling\_map}.insert\_pair(\textit{work\_op}, \textit{time\_op})\;
	}

	\textit{old\_work\_op} $\leftarrow$ 0\;
	\textit{old\_time\_op} $\leftarrow$ 0\;
	\ForEach{\normalfont$i$ in \textit{\textit{abnormal\_list}}}{
		
		\ForEach{\normalfont$batch$ in \textit{\textit{potential\_batch\_list}}}{
			
			\textit{work\_op} $\leftarrow$ getComputationWorkload($op_i$, batch)\;
			\textit{time\_op} $\leftarrow$ profileExecutionLatency($op_i$, batch)\;
			
			\If{ \textit{old\_work\_op} / \textit{work\_op} > \textit{old\_time\_op} / \textit{old\_time\_op} }{
					\textit{split\_plan}.insert\_tuple(i, $op_i$.batch/batch)\;
					\textbf{break}\;
			}
		
				\textit{old\_work\_op} $\leftarrow$ = \textit{work\_op}\;
				\textit{old\_time\_op} $\leftarrow$ = 	\textit{time\_op}\; 
			
		}
	}
	
\end{algorithm}

==> figure-DSP-inference.tex <==
\begin{figure}[t]
	\centering
	\subfigure[Inference time] {\includegraphics[width=0.22\textwidth]{figs/figure-inference-comparison-latency.pdf} } 
	\subfigure[Energy consumption]{\includegraphics[width= 0.22\textwidth ]{figs/figure-inference-comparison-power.pdf} }
	\vspace{-0.5cm}
	\caption{The inference time and energy consumption of different model precision (batch size = 64). The experiments are performed on XiaoMi 10 with TensorFlow Lite.} 
	\label{fig-inference-comparison}
	%\vspace{-1cm}
\end{figure}


==> figure-big-little.tex <==
\begin{figure}[t]
	\centering
	\subfigure[\textbf{VGG16}]{ \includegraphics[width=0.22\textwidth]{figs/figure-big-little-train-vgg16.pdf}  } 
	\caption{Training performance with Big/Liitle cores on different models.} 
	\label{fig-per-batch-latency}
\end{figure}

==> figure-parallel-execution.tex <==
\begin{figure}[t]
	\centering
	
	\includegraphics[width=0.48\textwidth]{figs/parallel-execution.pdf}
	
	\caption{ Parallel Execution. Subgraph in purple execute on CPU; while green on DSP} %图片标题
	\label{fig-parallel-execution}
\end{figure}

==> figure-rescale-split.tex <==
\begin{figure}[t]
	\centering
	
	\includegraphics[width=0.48\textwidth]{figs/intra-op-optimization.pdf}
	\vspace{-0.7cm}
	\caption{Self-adaptive rescaling and Batch splitting} %图片标题
	\label{fig-rescaling-split}
	\vspace{-0.5cm}
\end{figure}

==> sec-impl.tex <==
\section{Implementation}\label{sec:impl}
We have fully implemented \sys (15k LoC in C/C++ and 800 line  assembly codes in total) as a standalone framework supporting models exported from MNN \cite{mnn}, TFLite \cite{tflite}, and Pytorch Mobile \cite{pytorch}.
\sys leverages Hexagon NN \cite{hexagon-nn} as the DSP backend, which is the only  open-source library supporting inference on DSP developed by Qualcomm.
While \sys is compatible with different training algorithms, to demonstrate its efficiency, we use NITI~\cite{wang2020niti} as the default hybrid-precision training algorithm.
We use NITI because (i) it achieves the state-of-the-art convergence results; (2) it is a fully INT8 training algorithm therefore more suitable for DSP to execute.
\sys prototype contains four modules:
\begin{itemize}[leftmargin=0pt,itemindent=10pt,topsep=0pt]
\item \textbf{Translation engine that converts front-end models to intermediate model.}
We refer to different front-end models conversion logic in the MNN to implement our translation logic by further adding DSP operators (forward and backward) and DSP operators backpropagation rules.
During the translation process, \sys also runs profiling to determine whether a layer should split batch ($\S$~\ref{sec:splitting}). 
To simplify the translation process, a JSON file with ops' hyperparameters and dependencies is also generated so that \sys can directly use it to generate DSP training compute subgraphs without translation next time.

\item \textbf{Execution controller}
We implement three controllers  for self-adaptive rescaling ($\S$~\ref{sec:rescaling}), context-switching-aware parallel execution ($\S$~\ref{sec:parallel}), and compute graph reuse ($\S$~\ref{sec:reuse}), respectively. 
The three controllers are embedded into the execution engine in the form of plugins, and users can customize them.

\item \textbf{DSP training backend} is used to perform execute operators on DSP.
We have implemented common backward ops and forward ops with dynamic rescaling ($\S$~\ref{sec:rescaling}) for different training algorithms.
Since Hexagon DSP architecture is constantly changing and the backward compatibility is available since with V66 architecture (released in 2019), we mainly optimize our implementation for V66 architecture through assembly code.
Besides, for the convenience of debugging, each DSP operator has two mode: seperate and package.
In seperate mode, DSP operators execute one by one which is used for performance debugging; while package mode will merge DSP operators to compute subgraphs and execute them together.
Lastly, we also expand NITI algorithm to support element-wise ops, like matrix add, and implement them for DSP.

\item \textbf{CPU INT8 baseline.} 
We implement the baseline based on NITI as well to further illustrate our performance benefits.
Some operators implementation, like CONV and POOL are reused from MNN.
We also use NEON~\cite{reddy2008neon} assembly codes to optimize the performance of this baseline.
\end{itemize}

%Note that all of them above run on devices in an automated manner, imposing no additional efforts for developers.
%Besides, while \sys is conceptually compatible with both Android as well as iOS devices and DSP is common on smart phones, our system currently targets Android devices with Qualcomm Snapdragon SoCs as only Qualcomm Hexagon DSP support software usage.

%We use MNN because it outperforms TFLite \cite{tflite} and DL4J \cite{dl4j}, which are the only other two libraries that support training modern DNNs on Android devices.,in consideration of speed and memory usage as demonstrated in prior work \cite{cai2021towards}.
%Besides, 
%Lastly,  \cite{wang2020niti} is a fully INT8 training algorithm.
%Compared with other algorithms, it is simple and more suitable for DSP to execute.
%While MNN is conceptually compatible with both Android as well as iOS devices and DSP is common on smart phones, our prototype currently targets Android devices with Qualcomm Snapdragon SoCs as only Qualcomm Hexagon DSP support software usage.
%Except for \sys, we also implement  CPU low-precision training method based on \cite{wang2020niti} and MNN (around 5k LoC in C++ in total) as a baseline to further illustrate our performance benefits.
%
%
%MNN part (around 10k LoC in C++ in total) mainly includes two modules:
%(1) Generate and run DSP training computation subgraphs.
%Considering  training process needs both CPU and DSP, we choose to implement DSP operators (forward and backward) rather than a totally new DSP backend to solve compatibility issues, as well as DSP operators backpropagation rules.
%Thus, we can easily translate origin models to DSP ones and run them on DSP directly.
%During the translation process, we also controal whether a layer should split batch (Section~\ref{sec:splitting}). 
%Besides, each DSP operator has two mode: standalone and package.
%When standalone mode open, DSP operators execute one by one which is used for debugging; while package mode requires to merge DSP operators to compute subgraphs and execute them together.
%(2) Be responsible for parallel execution (Section~\ref{sec:parallel}) and compute graph reuse (Section~\ref{sec:reuse}).
%These two functions are embedded into the system in the form of plugins, and users  can customize them (open as default).
%Note that both of them run on devices in an automated manner, imposing no additional efforts for developers.
%
%Hexagon part (around 1.5k LoC in C and 800 line  assembly code in total) is used to perform DSP operators execution.
%We have implemented common backward ops and forward ops with dynamic rescaling (Section~\ref{sec:rescaling}) as well as fixed memory bugs.
%Since DSP architecture is constantly changing and only backward compatible starting with V66 (SoCs around 2019), we mainly optimize our implementation for V66 type by using assembly code.



==> tab-end-to-end-FL-settings.tex <==
\begin{table}[t]
%	\small
	\begin{tabular}{lrrr}
		\hline
		\textbf{Dataset \& Model} & \textbf{Batch size} & \textbf{Clients} & \textbf{Samples} \\ \hline
		CIFAR-10~VGG16 & 64 & 100 & 500 \\ \hline
		CIFAR-100~VGG16 & 64 & 500 & 100 \\ \hline
	\end{tabular}
	\caption{Federated learning settings.}
	\label{tab:fl-settings}
\end{table}
